Cyber risk and the cross-section of stock returns

We extract firms' cyber risk with a machine learning algorithm measuring the proximity between their disclosures and a dedicated cyber corpus. Our approach outperforms dictionary methods, uses full disclosure and not devoted-only sections, and generates a cyber risk measure uncorrelated with other firms' characteristics. We find that a portfolio of US-listed stocks in the high cyber risk quantile generates an excess return of 18.72% p.a. Moreover, a long-short cyber risk portfolio has a significant and positive risk premium of 6.93% p.a., robust to all factors' benchmarks. Finally, using a Bayesian asset pricing method, we show that our cyber risk factor is the essential feature that allows any multi-factor model to price the cross-section of stock returns.

==> backups/literature_review.tex <==

\subsection{Natural language processing in finance}

\subsubsection{Dictionary approach}

\subsubsection{10-K statements}

\subsubsection{Machine learning}



\subsection{Economic implications of cyber risk}

\subsection{Cybersecurity costs}
\subsubsection{Direct estimations}

%Define RQ, contribution
\cite{AndersonBartonBöhmeClaytonEetenLeviMooreSavage2013} perform a systematic study of the costs of cybercrime. They differentiate direct, indirect, and defense costs and disentangle the different types of cybercrimes. They find that traditional crimes that are conducted online, such as tax and welfare fraud, cost the typical citizen hundreds of dollars per year. Transitional crimes, such as credit card fraud, cost a few dollars a year, while new crimes, such as the provision of botnets, cost tens of cents a year. Indirect and defense costs, however, are much higher for transitional and new crimes. They conclude that we should spend less anticipating cybercrime and more in response.

\cite{AndersonBartonBöhmeClaytonGananGrassoLeviMooreVasek2019} revisit the previous study. They observe that even though payment frauds have doubled over the seven years separating the initial studies, their average costs for the citizens have fallen. They conclude that economic optimality would be spending less on cyberattack prevention and more on response and law enforcement. \cite{Bouveret2018W} documents cyber risk worldwide in the financial sector by analyzing the different types of cyber incidents and identifying patterns. He uses a Value at Risk (VaR) type of framework. He finds an average loss due to cyberattacks of USD 97 bn at the country level and a VaR between USD 147 and 201 bn. He concludes that there are sizeable potential aggregated losses in the financial sector, several orders of magnitude higher than the cyber insurance market can cover. \cite{Romanosky2016}) studies the composition and costs of cyber events. After analyzing a sample of over 12,000 cyber events, he finds that the cost distribution is heavily skewed, with an average cost of USD 6 mln and a median cost of USD 170,000 (comparable to the firm's annual IT security budget). He concludes that with these relatively low costs, firms may be engaging in a privately optimal level of security. Subsequently, firms are investing in only a modest amount of data protection.

\subsubsection{Indirect estimations with municipal bonds}

\cite{AndreadisKalotychouLoucaLundbladMakridis2023} study the impact of information dissemination about cyberattacks through significant news sources on municipalities' access to finance, focusing on the municipal bond market. They employ a difference-in-differences framework and find that the cumulative number of cyberattacks covered by county-level news articles and the corresponding number of county-level cyberattack news articles significantly adversely affect municipal bond yields. A 1\% increase in the number of cyberattacks covered by news articles leads to an increase in offering yields ranging from 3.7 to 5.9 basis points, depending on the level of attack exposure (number of significant cyberattack news in the county). \cite{JensenPaine2023} perform a similar analysis, using data about municipal IT investment, ransomware attacks, and bonds. They find no immediate effect on bond yields of hacked towns in a 30-day window around a hack. In the 24 months following a ransomware attack, they find that the municipal bond yields gradually declined and IT spending increased. They argue that the declining bond yields are driven by a decrease in the town's cyber risk due to increased IT spending.

\subsubsection{Indirect estimations with stock price reaction}

\cite{GordonLoebZhou2011} study the impact of information security breaches on stock returns by computing the cumulative abnormal returns on a three-day event window centered on newspaper reports of cybersecurity incidents. They find that news about information security breaches had a statistically significant effect on the stock returns of publicly traded firms. They also show that there has been a significant downward shift in the impact of security breaches in the post-9/11 period. The findings from the study suggest that in recent years, average information security breaches have become less costly, and there seems to be a shift in attitude among investors toward viewing information security breaches as creating a corporate \quotes{nuisance} rather than a potentially serious economic threat. In a similar study, \cite{CampbellGordonLoebZhou2003} find a highly significant negative market reaction for information security breaches involving unauthorized access to confidential data but no significant reaction when the breach does not include confidential information.
\cite{JohnsonKangLawson2017} also study cumulative abnormal returns around cyber security events. They show that, on average, publicly traded firms in the U.S. lost 0.37\% of their equity value when a data breach occurs. Breaches resulting from payment card fraud contribute more to negative announcement returns than the other breach types, and the adverse effects are more important for firms with card breaches more significantly than the average. For the average firm, these breaches result in a 3\% decline in firm equity value.

\cite{LendingMinnickSchorno2018} study the relationship between corporate governance, social responsibility, and the probability of data breaches, and they measure the changes in stock returns following data breaches. They find that the financial impact of a breach is visible in the long term, as data-breach firms have –3.5\% one-year buy-and-hold abnormal returns. They also find that banks with breaches have significant declines in deposits, and non-banks have substantial declines in sales in the long run. \cite{Tosun2021} studies how financial markets react to unexpected corporate security breaches in the short and long run. He finds that the market reaction regarding trading volume, liquidity, and selling pressure anticipates negative changes in stock prices, which are significant and negative only the day after security breaches are publicly announced. He also finds that cyberattacks affect firms’ policies in the long run. He concludes that security breaches represent unexpected adverse shocks to firms’ reputations. \cite{KamiyaKangKimMilidonisStulz2021} also find evidence of a reputation loss for target firms in the form of a decrease in credit ratings or decreased sales growth.

\subsubsection{Indirect estimations with disclosures}

\cite{GordonLoebSohail2010} assess the market value of voluntary information security disclosures of firms, using a sample of 1,641 disclosing and 19,266 non-disclosing firm-year observations. They argue that voluntary disclosures about information security could mitigate potential litigation costs and lower the firm's cost of capital by reducing the information asymmetry between a firm's management and its investors. They find a positive association of the voluntary disclosure variable with firm value, and the bid-ask spread for firms that provide voluntary disclosures of information security is statistically lower than for firms not providing such disclosure. \cite{HilarySegalZhang2016W} also study cyber risk disclosures. They find that the market reaction to cyber breaches is statistically significant but economically limited.

\cite{FlorackisLoucaMichaelyWeber2023} build a text-based cyber risk score using a section of 10-K statements called \quotes{Item 1.A Risk Factors}. They extract cyber risk-related sentences from this section of the statements using a list of keywords and restrict the analysis to these sentences. They consider recently hacked firms as a training sample and compute the cybersecurity exposure of firms as the average similarity between the bag-of-words representation (vector of the number of occurrences of each word in their dictionary) of the firm's cybersecurity sentences and the cybersecurity sentences of the training sample. They find that stocks with high exposure have higher returns on average but perform worse in periods of cyber risk. \cite{JamilovReyTahoun2021W} perform a similar analysis using quarterly earnings calls. They construct the cyber risk score using the frequency of cybersecurity-related keywords in the earnings calls. They build a cybersecurity factor by first computing the monthly average cyber risk score of the subset of firms with non-zero scores and then fitting an $AR(1)$ model to the time series and extracting the residuals. This factor captures the shocks to cyber risk. They find a factor structure in the firm-level measure of cybersecurity: the long-short portfolio built on cybersecurity beta sorted portfolios has an average annual return of -3.3\% (the negative sign is because the factor captures shocks to cybersecurity).

We are only aware of four studies focusing on cyber risk and its factor structure using disclosures). However, these studies employ a dictionary approach that leaves many firm-year observations with a cyber risk of zero (71\% of firms in 2007 in the case of \cite{FlorackisLoucaMichaelyWeber2023} and over 98\% of earnings calls in 2007 in the case \cite{JamilovReyTahoun2021W}).\footnote{See also, \citealp{JiangKhannaYangZhou2023,LiuMarshXiao2022W}} Furthermore, this approach does not consider the context of the keywords, only their presence in the disclosures. We use the \quotes{Paragraph Vector} algorithm to fill this gap to build a cyber risk score using firms' 10-K statements. Hence, we define our hypotheses as follows:

% check if florackis have a forward-looking bias or that what they estimate is not a measure of recovery post-cyberattack

%\begin{itemize}
%    \item $H_1$ The cyber risk is not priced       in the cross-section of stock returns.

    %Score/estimate:
    %- uncorrelated with other properties
    %- capturing all content (not only item 1-A).
    %- capturing context, not only words
    %- does not generate zero-risk
    %- capturing missed paragraphs
    
    %- Cyber risk measure is not biased by cybersecurity-providing firms

    %Is robustness to other factors enough to be a hypothesis?

    %- Cyberfactor is essential to price the cross-section of returns. (Barillas and Shanken corresponding test).

    %%%%%%%%%%%%%
    %add more hyp. based on what we have, 
    %add a comment on results comparing with former research
    %comment hyp. rejection in the Results section.
%\end{itemize}

\subsection{Vector representation of paragraphs}

\cite{LeMikolov2014} develop an unsupervised algorithm called \quotes{Paragraph Vector} that can learn fixed-length vector representations from variable-length pieces of texts, such as sentences, paragraphs, and documents. For example, each piece of text is represented by a dense vector that can be used for text classification and sentiment analysis. The advantage of this algorithm over other methods, such as bag-of-words, is that it learns the semantics of words and sentences. \cite{LauBaldwin2016} perform a rigorous empirical evaluation of this algorithm and provide recommendations on hyper-parameter settings for general-purpose applications. \cite{AdosoglouLombardoPardalos2021} use the \quotes{Paragraph Vector} algorithm with financial filings (10-K statements). They construct portfolios based on the semantic differences between two consecutive financial reports of each firm. They find that cosine similarity is the most effective metric for neural network embeddings, such as the ones obtained using the \quotes{Paragraph Vector} algorithm.



%%%%%%% Jiang et al 2023:
%- count the number of cyber words in Item 1A (cyber dictionary taken from NIST)
%- combine the previous count with firm characteristics (from Kamiya et al 2021) into a logit ridge regression with the output being the realization of a cyberattack (fit the model for each year using all the previous years as training data)
%- they choose cyberattacks that have a [-3,3] day CAR above 1% (394 events in total)
% (=> highly unbalanced regression, can correctly predict cyberattacks 50% of the time)
%- only show long-short alphas which are ~ 0.8% (CAPM) to 0.5% (FF6) per month
%- long-short portfolio is negatively correlated with cyber ETFs (-0.405 and -0.312)

%%%%%%% Liu et al 2022:
%- uses intertemporal CAPM and cybercrime news attention (compute betas wrt the Thomson-Reuters MarketPsych (TRMI) cybercrime news index)
%- they find that high cybercrime-beta stocks generate 0.6% lower returns than low cybercrime-beta stocks
%- they argue their method is better as their high beta stocks could act as hedges to cyber risk (instead of low-risk stocks)

%Jamilov 2021... not anymore.
%They build a cybersecurity factor by first computing the monthly average cyber risk score of the subset of firms with non-zero scores and then fitting an $AR(1)$ model to the time series and extracting the residuals. This factor captures the shocks to cyber risk. They find a factor structure in the firm-level measure of cybersecurity: the long-short portfolio built on cybersecurity beta sorted portfolios has an average annual return of -3.3\% (the negative sign is because the factor captures shocks to cybersecurity).



%\cite{CohenMalloyNguyen2020} lazy prices paper. changes in 10-K. interesting for a pure disclosure lit. review.
%\cite{CampbellChenDhaliwalLuSteele2014}% again, about disclosures and the mandatory risk section of them.




\cite{JegadeeshWu2013} %and present a new approach for content analysis to quantify document tone. We find a significant relation between our measure of the tone of 10-Ks and market reaction for both negative and positive words. We also find that the appropriate choice of term weighting in content analysis is at least as important as, and perhaps more important than, a complete and accurate compilation of the word list. Furthermore, we show that our approach circumvents the need to subjectively partition words into positive and negative word lists. Our approach reliably quantifies the tone of IPO prospectuses as well, and we find that the document score is negatively related to IPO underpricing.

\cite{Garcia2013} %studies the effect of sentiment on asset prices during the 20th century (1905 to 2005). As a proxy for sentiment, we use the fraction of positive and negative words in two columns of financial news from the New York Times. The main contribution of the paper is to show that, controlling for other well-known time-series patterns, the predictability of stock returns using news’ content is concentrated in recessions. A one standard deviation shock to our news measure during recessions predicts a change in the conditional average return on the DJIA of 12 basis points over one day.

\cite{CalomirisMamaysky2019} %develop a classification methodology for the context and content of news articles to predict risk and return in stock markets in 51 developed and emerging economies. A parsimonious news summary, including topic-specific sentiment, frequency, and unusualness (entropy) of word flow, predicts future country-level returns, volatilities, and drawdowns. Economic and statistical significance are high and larger for year ahead than monthly predictions. The effect of news measures on market outcomes differs by country type and over time. News stories about emerging markets contain more incremental information. Out-of-sample testing confirms the economic value of our approach for forecasting country-level market outcomes.

\cite{BodnarukLoughranMcDonald2015} %measure the extent to which a firm is financially constrained is critical in assessing capital structure. Extant measures of financial constraints focus on macro firm characteristics such as age and size, variables highly correlated with other firm attributes. We parse 10-K disclosures filed with the U.S. Securities and Exchange Commission (SEC) using a unique lexicon based on constraining words. We find that the frequency of constraining words exhibits very low correlation with traditional measures of financial constraints and predicts subsequent liquidity events, such as dividend omissions or increases, equity recycling, and underfunded pensions, better than widely used financial constraint indexes.

%not positive/negative but disagreement to determine volume.
\cite{AntweilerFrank2004} %study the effect of more than 1.5 million messages posted on Yahoo! Finance and Raging Bull about the 45 companies in the Dow Jones Industrial Average and the Dow Jones Internet Index. Bullishness is measured using computational linguistics methods. Wall Street Journal news stories are used as controls. We find that stock messages help predict market volatility. Their effect on stock returns is statistically significant but economically small. disagreement among the posted messages is associated with increased trading volume.

%word count and bigram counts frequency, for political risk. 
\cite{HassanHollandervLentTahoun2019} %adapt simple tools from computational linguistics to construct a new measure of political risk faced by individual U.S. firms: the share of their quarterly earnings conference calls that they devote to political risks. We validate our measure by showing that it correctly identifies calls containing extensive conversations on risks that are political in nature, that it varies intuitively over time and across sectors, and that it correlates with the firm’s actions and stock market volatility in a manner that is highly indicative of political risk. Firms exposed to political risk retrench hiring and investment and actively lobby and donate to politicians. These results continue to hold after controlling for news about the mean (as opposed to the variance) of political shocks. Interestingly, the vast majority of the variation in our measure is at the firm level rather than at the aggregate or sector level, in the sense that it is captured neither by the interaction of sector and time fixed effects nor by heterogeneous exposure of individual firms to aggregate political risk. The dispersion of this firm-level political risk increases significantly at times with high aggregate political risk. Decomposing our measure of political risk by topic, we find that firms that devote more time to discussing risks associated with a given political topic tend to increase lobbying on that topic, but not on other topics, in the following quarter.

%also bigram approach combined with positive/negative. claim to use an "algorithm" but its not, an ML one, rather a procedure.
\cite{SautnerLentVilkovZhang2023} %develop a method that identifies the attention paid by earnings call participants to firms’ climate change exposures. The method adapts a machine learning keyword discovery algorithm and captures exposures related to opportunity, physical, and regulatory shocks associated with climate change. The measures are available for more than 10,000 firms from 34 countries between 2002 and 2020. We show that the measures are useful in predicting important real outcomes related to the net-zero transition, in particular, job creation in disruptive green technologies and green patenting, and that they contain information that is priced in options and equity markets.

%proximity in the language used in 10-K indicators of frequency of mergers or acquisitions
\cite{HobergPhillips2010} %use text-based analysis of 10-K product descriptions to examine whether firms exploit product market synergies through asset complementarities in mergers and acquisitions. Transactions are more likely between firms that use similar product market language. Transaction stock returns, ex-post cash flows, and growth in product descriptions all increase for transactions with similar product market language, especially in competitive product markets. These gains are larger when targets are less similar to acquirer rivals and when targets have unique products. Our findings are consistent with firms merging and buying assets to exploit synergies to create new products that increase product differentiation.

==> backups/tables_and_figures.tex <==

%Fama-MacBeth with weighted dummies.
\clearpage
\begin{table}
\vspace{-2em}
\begin{adjustbox}{width=0.77\textwidth,center}
    \noindent\makebox[\textwidth]{%
    \begin{tabular}{llllllll}
    \toprule
    \toprule
    \multicolumn{8}{c}{Monthly Portfolio returns}\\
    \midrule
    & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{1}{c}{(6)} & \multicolumn{1}{c}{(7)}\\
    \midrule
    $\beta_{Market}$ & \textbf{-0.005} & & \textbf{-0.025} & \textbf{0.065}  & \textbf{0.024} & & \textbf{-0.033}\\
    & [-0.064] & & [-0.429] & [0.997] & [0.275] & & [-0.578]\\
    Cyber risk & & \textbf{0.183}$^{*}$& \textbf{0.182}$^{**}$ & \textbf{0.183}$^{*}$ & \textbf{0.172}$^{**}$ & \textbf{0.156}$^{*}$ & \textbf{0.176}$^{**}$\\
    & & [1.794] & [1.994] & [1.913] & [2.037] & [1.951] & [2.103]\\
    $\beta_{HML}$ & & & & \textbf{0.027} & \textbf{-0.012} & \textbf{-0.116} & \textbf{-0.033}\\
    & & & & [0.439] & [-0.126] & [-1.236] & [-0.293]\\
    $\beta_{SMB}$ & & & & \textbf{0.069}  & \textbf{0.049} & \textbf{0.200} & \textbf{-0.042}\\
    & & & & [0.835] & [0.536] & [0.951] & [-0.385]\\
    $\beta_{MOM}$ & & & & \textbf{0.011} & & &\\
    & & & & [0.153] & &\\
    $\beta_{RMW}$ & & & & & \textbf{-0.085} & \textbf{0.062} & \textbf{-0.086}\\
    & & & & & [-1.436] & [0.753] & [-1.150]\\
    $\beta_{CMA}$ & & & & & \textbf{-0.088} & \textbf{-0.173} & \textbf{0.011}\\
    & & & & & [-0.816] & [-0.925] & [0.076]\\
    \\
    Consumer Durables & & & & & & \textbf{-0.013}\\
    & & & & & & [-0.212]\\
    Manufacturing & & & & & & \textbf{-0.094}\\
    & & & & & & [-1.261]\\
    Energy & & & & & & \textbf{0.059}\\
    & & & & & & [0.645]\\
    Chemicals & & & & & & \textbf{0.062}\\
    & & & & & & [0.909]\\
    Telecommunications & & & & & & \textbf{-0.162}$^{**}$\\
    & & & & & & [-2.190]\\
    Retail & & & & & & \textbf{0.139}\\
    & & & & & & [1.272]\\
    Healthcare & & & & & & \textbf{-0.003}\\
    & & & & & & [-0.046]\\
    Finance & & & & & & \textbf{-0.019}\\
    & & & & & & [-0.211]\\
    Constant & \textbf{1.445}$^{***}$ & \textbf{1.465}$^{***}$ & \textbf{1.457}$^{***}$ & \textbf{1.455}$^{***}$ & \textbf{1.476}$^{***}$ & \textbf{1.329}$^{***}$ & \textbf{1.362}$^{***}$\\
    & [5.311] & [5.540] & [5.493]& [5.413] & [5.450] & [4.081] & [5.015]\\
    \midrule
    $\overline{R2_{adj}}$ & 0.007 & 0.134 & 0.186 & 0.258 & 0.284 & 0.307 & 0.295\\
    MAPE & 1.360 & 1.312 & 1.233 & 1.064 & 0.987 & 0.636 & 1.243\\
    Nb portfolios & 20 & 20 & 20 & 20 & 20 & 20 & 31 \\
    \hline
    \hline
    \end{tabular}}
    \end{adjustbox}
    \caption{\textbf{Fama-MacBeth regressions}}\bigskip
    \footnotesize{This table reports the results of Fama-MacBeth regressions of 20 value-weighted portfolios sorted on their cyber risk. In Specification (7), we extend the set of test assets with an additional 11 industry portfolios. These portfolios are regressed each month on portfolio value-weighted betas with the market, HML, SMB, MOM, RMW, and CMA, as well as on industry dummies in Specification (6). \quotes{Cyber risk} is the value-weighted cyber-risk of each portfolio. The betas are standardized before the second step-regressions and estimated with a two-year rolling window. HML and SMB refer to the book-to-market and size factors from \cite{FamaFrench1992}. MOM refers to the momentum factor from \cite{Carhart1997}. CMA and RMW refer to the investment and operating profitability factors from \cite{FamaFrench2015}. $\overline{R2_{adj}}$ is the average adjusted R-squared, and MAPE is the mean average pricing error. Newey-West t-statistics are reported in brackets. $^{*}$, $^{**}$, and $^{***}$ indicate significance at the 10\%, 5\% and 1\% levels, respectively. The period is from January 2009 to December 2022.}
    \label{tab:Fama_MacBeth}
\end{table}
